Discrete-Time Periodic Monotonicity Preserving Systems

Two nested classes of discrete-time linear time-invariant systems, which differ by the set of periodic signals that they leave invariant, are studied. The first class preserves the property of periodic monotonicity (period-wise unimodality). The second class is invariant to signals with at most two sign changes per period, and requires that periodic signals with zero sign changes are mapped to the same kind. Tractable characterizations for each system class are derived by the use and extension of total positivity theory via geometric interpretations. Central to our results is the characterization of sequentially convex contours via consecutive minors. Our characterizations also extend to the loop gain of Lur'e feedback systems as the considered signals sets are invariant under common static non-linearities, e.g., ideal relay, saturation, sigmoid function, quantizer, etc. The presented developments aim to form a base for future signal-based fixed-point theorems towards the prediction of self-sustained oscillations. Our examples on relay feedback systems indicate how periodic monotonicity preservation gives rise to useful insights towards this goal.

==> sec_main.tex <==
\section{Monotone Frequency Response Gains}
The main objective of this paper is to exploit the properties of $g(t)$ and $R_{gg}(t)$ in order to characterize monotonicity properties of the system gain $|G(i\omega)|$. In this section, we often omit the period $T$ from the notation of the PM and PMP properties, as they will be clear from context. 

\subsection{PMP and the frequency response gain}

We begin with a technical lemma:
\begin{lem}\label{lem:input}
For $\omega > 0$ and $k \in \mathds{N}_{>0}$, there exists an $a > 0$ such that $u = \sin(\omega t) - a\sin(k \omega t)$ is $\text{PMP}_{2\pi/\omega}$. 
	
\end{lem}

\begin{proof}
It suffices to show the claim for $\omega = 1$ as scaling of $t$ leaves the claim invariant. By \cref{lem:CC}, we need to show then that there exists an $a > 0$ such that
\begin{align*}
\small  M := \det \begin{pmatrix}
        1 & \sin(t_1) - a\sin(kt_1) &  \cos(t_1) - ak\cos(kt_1)\\
        1 & \sin(t_2) - a\sin(kt_2) &  \cos(t_2) - ak\cos(kt_2)\\
        1 & \sin(t_3) - a\sin(kt_3) &  \cos(t_3) - ak\cos(kt_3) 
    \end{pmatrix} 
\end{align*}
has the same non-zero sign for all $t_1 < t_2 < t_3 < t_1 + 2\pi$. To verify this, we note that
\begin{align*}
    M &= \begin{pmatrix}
        1 & \sin(t_1) &  \cos(t_1) \\
        1 & \sin(t_2)  &  \cos(t_2)\\
        1 & \sin(t_3) &  \cos(t_3)
    \end{pmatrix} + \mathcal{O}(a) \\
    &= 4 \sin\left(\frac{t_1-t_2}{2}\right)\sin\left(\frac{t_2-t_3}{2}\right)\sin\left(\frac{t_1-t_3}{2}\right) + \mathcal{O}(a)
\end{align*}
with
\begin{align*}
    0 &> \frac{t_1-t_2}{2} > -\pi, \quad 0 > \frac{t_1-t_3}{2} > -\pi,\\ 
    0 &> \frac{t_2-t_3}{2} > \frac{t_1-t_3}{2} > -\pi.
\end{align*}
Thus, $M < 0$ for sufficiently small $a > 0$.
\end{proof}

Our first main result is the following:
\begin{thm}\label{thm:main}
    Let $\omega > 0$ be such that $\psumauto{\frac{2 \pi}{\omega}}$ is PMP. Then, $|G(i \omega)| \geq |G(i  k \omega)|$ for all $k \in \mathds{N}_{\geq 1}$.
\end{thm}
\begin{proof}
    By \cref{lem:input}, there exists an $a>0$ such that $u_a(t) = \sin(\omega t) - a\sin(k\omega t)$ {\color{black}is PMP}. Let $\bar{a}$ be the largest such $a$. It is easy to see that $\bar{a} < \infty$, because for sufficiently large $a$, $u_a(t)$ will be dominated by $\sin(k \omega t)$ and, then $u$ is no longer PM. It follows from \cref{eq:freq_resp_auto} that
     \begin{equation*}
     	(R_{gg} \ast u_{\bar{a}})(t) = |G(i \omega )|^2\sin(\omega t) - \bar{a} |G(i k  \omega)|^2 \sin(k  \omega t). \label{eq:montone_gain}
    \end{equation*}
Since $R^{\frac{2\pi}{\omega}}_{gg}$ is PMP by assumption, and $u_{\bar{a}}$ is PMP by \cref{lem:input}, then \cref{lem:pmp_facts} implies that 
\begin{equation*}
u_{b}=|G(i \omega )|^{-2}(R_{gg} \ast u_{\bar{a}}),
\quad b=\bar{a}\frac{|G(ik\omega)|^2}{|G(i\omega)|^2}
\end{equation*}
is PMP. {\color{black}But since we have chosen $\bar{a}$ to be the largest $a$ such that $u_a$ is PMP, $u_b$ can only be PMP if $\frac{|G(i k\omega)|}{|G(i \omega)|} \leq 1$.}
\end{proof}
If $\psumauto{T}$ is PMP for all $T = \frac{\pi}{2^{k-1} \omega} > 0$, $k \in \mathds{Z}$, then \cref{thm:main} indicates a monotonic gain decrease:
\begin{equation*}
    |G(i2^k \omega)| \geq |G(i2^{k+1}\omega)|, \; k \in \mathds{Z}.
\end{equation*}
It can be shown that the above also applies to LTI systems that preserve the PM$_T$ property of their inputs:
\begin{prop}
    \label{prop:sufficient_Rgg}
    Let $g^{T}$ be PMP$_T$. Then, $R_{gg}^T$ is PMP$_T$.
\end{prop}
\begin{proof}
    Analogously to what is done in \cite[p. 264]{karlin1968total}, we use \eqref{eq:periodized_relation} to write the cyclic convolution \eqref{eq:periodic_convolution} as the composition of two cyclic convolutions involving $g^{T}$. Namely, a few simple manipulations show that $R_{gg}^T \ast u =  (g^T \ast g^T_-) \ast u$, where $g^T_-(t) := g^T(-t)$. 
    By \cref{lem:pmp_facts}, it follows that both $g^T_- \in \text{PMP}_T$ and $R_{gg}^T \in \text{PMP}_T$.
\end{proof}

Unfortunately, at present it is not known whether the converse of \cref{prop:sufficient_Rgg} holds. For this reason, in the rest of the section we focus on analyzing the periodized autocorrelation, which provides the most general way of obtaining the sampled frequency response monotonicity property above.

Next, we would like to provide conditions that allow us to apply \cref{thm:main}. We begin by the PM condition on  $\psumauto{\frac{2 \pi}{\omega}}$.
\begin{lem}
The following relationships between $\psumauto{T}$ and $R_{gg}$ hold:
\begin{enumerate}[i.]
    \item $\psumauto{T}(t)$ is convex on $[0,T)$ for all $T >0$ if and only if $R_{gg}$ is convex on $\mathds{R}_{\geq 0}$. 
    \item $\psumauto{T}(t)$ is log-concave on $[0,T)$ for all $T>0$ if and only if $R_{gg}$ is log-concave on $\mathds{R}_{\geq 0}$. 
\end{enumerate}
In particular, $\psumauto{T}(t)$ is PM in both cases. \label{lem:PM}
\end{lem}

\begin{proof}
We only need to show the sufficiency part, as the properties of $R_{gg}$ follow from those of $R_{gg}^T$ by taking $T \to \infty$.  

In the first claim, if $R_{gg}$ is convex on $\mathds{R}_{\geq 0}$, then $\sum_{k=0}^\infty R_{gg}(t+kT)$ is convex on $[0,T)$ since it is an infinite sum of convex functions on that interval \cite[Section 3.2.1]{boyd2004convex}. Since $R_{gg}$ is even, it is convex on $\mathds{R}_{\leq 0}$, and hence $\sum_{k=1}^\infty R_{gg}(t-kT)$ is also convex on $[0,T)$. Hence $\psumauto{T}(t) = \sum_{k=1}^\infty R_{gg}(t-kT) + \sum_{k=0}^\infty R_{gg}(t+kT)$ is convex on $[0,T)$. 

For the second claim, assume that $R_{gg}$ is log-concave on $\mathds{R}_{\geq 0}$. Then by \cref{lem:logconcave} in \cref{app:auxiliary} we have
\begin{align*}
     \det \begin{pmatrix}
      R_{gg}(t+iT) &  R_{gg}(t-h+jT)\\
      R_{gg}(t+h+iT) &  R_{gg}(t+jT)
  \end{pmatrix} \geq 0, i \leq j
\end{align*}
and
\begin{align*}
     \det \begin{pmatrix}
      R_{gg}(t+jT) &  R_{gg}(t-h+jT)\\
      R_{gg}(t+h+iT) &  R_{gg}(t+iT)
  \end{pmatrix} \geq 0, i > j
\end{align*}
for all $h > 0$ and $t$. Thus, 
\small{\begin{align*}
\det &\begin{pmatrix}
      \sum_{k=-\infty}^\infty R_{gg}(t+kT) &  \sum_{k=-\infty}^\infty R_{gg}(t-h+kT)\\
         \sum_{k=-\infty}^\infty  R_{gg}(t+h+kT) &  \sum_{k=-\infty}^\infty  R_{gg}(t+kT)
  \end{pmatrix} \\
  &=\sum_{i=-\infty}^\infty \sum_{j=-\infty}^\infty  \det \begin{pmatrix}
      R_{gg}(t+iT) &  R_{gg}(t-h+jT)\\
      R_{gg}(t+h+iT) & R_{gg}(t+jT)
  \end{pmatrix}
\end{align*}} \normalsize
is nonnegative for all $h > 0$ and $t+h \in [0,T)$. This is equivalent to $\psumauto{T}$ being log-concave on $[0,T)$ by \cref{lem:logconcave} in \cref{app:auxiliary}.

In particular, as convex and log-concave functions are unimodal, $\psumauto{T}(t)$ is PM for both cases.
\end{proof}
 Note that while both cases of \cref{lem:PM} deal with a unimodal $R_{gg}$, unimodality is in general not sufficient to claim PM of $R_{gg}^T$.

Analogously to the second claim in \cref{lem:PM}, the following relationship for $\dot{R}_{gg}^T$ will allow us to verify the third item in \cref{prop:pmp}.
\begin{lem}\label{lem:deriv_log}
$|\dot{R}_{gg}^T|$ is log-concave on $(0,T)$ for all $T >0$ if and only if $|\dot{R}_{gg}|$ is log-concave on $\mathds{R}_{> 0}$.
\end{lem}
\begin{proof}
The necessity follows from taking $T \to \infty.$ 
To see the sufficiency, first notice that if $|\dot{R}_{gg}|$ is log-concave on $\mathds{R}_{> 0}$, then $\dot{R}_{gg}$ cannot change sign, since in that case $|\dot{R}_{gg}|$ would not even be unimodal on $\mathds{R}_{> 0}$. Hence $\dot{R}_{gg}\ge 0$ or $\dot{R}_{gg}\le 0$ for all $t \ge 0$. But since $R_{gg}(0) = \|g\|_{\mathcal{L}_2}^2 > 0$, it is the latter that must hold. Hence, the log-concavity of  $|\dot{R}_{gg}|$ on $\mathds{R}_{> 0}$ is equivalent to log-concavity of $-\dot{R}_{gg}$ on that interval. Hence, 
\begin{align*}
     \det \begin{pmatrix}
      \dot{R}_{gg}(t+iT) &  \dot{R}_{gg}(t-h+jT)\\
      \dot{R}_{gg}(t+h+iT) &  \dot{R}_{gg}(t+jT)
  \end{pmatrix} \geq 0, i \leq j
\end{align*}
and 
\begin{align*}
     \det \begin{pmatrix}
      \dot{R}_{gg}(t+jT) &  \dot{R}_{gg}(t-h+jT)\\
      \dot{R}_{gg}(t+h+iT) &  \dot{R}_{gg}(t+iT)
  \end{pmatrix} \geq 0, i > j
\end{align*}
for all $h > 0$, $t+h \in (0,T)$ and $i,j \in \mathds{N}_0$. Further, these inequalities are also true for $-i,-j \in \mathds{N}$ by the evenness of $R_{gg}$. Analogously to the proof of the second claim in \cref{lem:PM}, it follows then that $|\dot{R}_{gg}^T|$ is log-concave on $(0,T)$. 
\end{proof}
Note that $R_{gg}^T$ is continuous on $[0,T]$ and smooth on $(0,T)$. For the cases of \cref{lem:PM}, the evenness of $R_{gg}^T$ then shows that $\sup_{t} R_{gg}^T(t) = R_{gg}^T(0)$. Thus, in conjunction with \cref{lem:PM,lem:deriv_log}, all items of \cref{prop:pmp} are fulfilled. This yields our next main result.  

\begin{thm}\label{thm:PMP_Rgg}
     Let $(A,b,c)$ be such that 
     \begin{equation}
         \ddot{R}_{gg}^2(t) \geq \dot{R}_{gg}(t) \dddot{R}_{gg}(t) \text{ for }t \in \mathds{R}_{> 0} \label{eq:log_conv_der}
     \end{equation}
     and either of the following two conditions hold:
     \begin{enumerate}[i.]
         \item $\ddot{R}_{gg}(t) \geq 0$ for all $t \in \mathds{R}_{\geq 0}$ \label{item:convex}
         \item $R_{gg}(t) > 0$ and $\dot{R}_{gg}^2(t) \geq R_{gg}(t) \ddot{R}_{gg}(t)$ for all $t \in \mathds{R}_{\geq 0}$ \label{item:log_conv}
     \end{enumerate}
     Then, $R_{gg}^T$ is PMP for all $T > 0$.
\end{thm}
In the next section, we will illustrate \cref{thm:PMP_Rgg} by analytical examples and discuss why its conditions are often computationally tractable.

\subsection{Variation diminishment and the frequency response gain}

In order to close the gap between the frequencies $2^j \omega$ and $2^{j+1}\omega$, we would require a generalization of the PMP property to signals with $\max_{\gamma} \varic{u-p\gamma \mathbf{1}} \leq 2k$, $k > 1$. At the present moment, we are not aware of such a generalization. 

An alternative is given by the CVD$_{2k}$ property (see \cref{def:cvd}). It has been shown by Karlin that a CVD$_{2k}$ kernel satisfies a different type of frequency response gain monotonicity with regards to that of \cref{thm:main}; see \cite[Lemma 5.7.2]{karlin1968total}. Unfortunately, working with $\text{CVD}_{2k}$ comes with two major drawbacks:
\begin{enumerate}
    \item $\text{CVD}_2$ is more restrictive than PMP \cite[pp.131-132]{ruscheweyh1992preservation}.
    \item Computationally verifiable conditions such as \cref{prop:pmp} seem to be unknown at this point. 
\end{enumerate}

An interesting special case of $\text{CVD}_0$ is the following sufficient condition for positive domination based on $R_{gg}$. 

\begin{prop}\label{prop:pos_dom}
Let $(A,b,c)$ be such that $(A,Pc^\transp,c)$ is externally positive, where $AP + PA^\transp = -bb^\transp$. Then $(A,b,c)$ is positively dominated.
\end{prop}
\begin{proof}
For $u(t) = 1 - \sin(\omega t)$, it follows by \cref{eq:freq_resp_auto,eq:auto_real} that $(R_{gg} \ast u)(t) = |G(0)|^2 - |G(i \omega)|^2 \sin(\omega t)$. 
Then, if $(A,Pc^\transp,c)$ is externally positive, $(R_{gg} \ast u)(t)$ is nonnegative, because $u$ and $R_{gg}$ are nonnegative. Taking $t = \frac{\pi}{2\omega}$ proves that $G$ is positively dominated. 
\end{proof}


  

















==> sec_pos.tex <==
\section{Convex Contours}
\label{sec:convex_contour}
In this section we present our first main result on the tractable characterization of so-called sequentially convex contours. This is a crucial intermediate result in preparation for our certificates of $\Conv{g}$ belonging to $\text{(S)}\pmp{T}$, $\text{(S)}\cvd{2}(T)$ or $\text{(S)}\cvd{2}(T)$. Our result also establishes a natural generalization of \cref{prop:karlin_scm} in case of $m=3$ and raises the non-trivial open question of extensions for $m > 3$. 

\subsection{Monotonicity \& Convexity}
We begin by showing that for $m = 2$ and $m=3$, \cref{prop:karlin_scm} follows from the locality properties of monotonicity and convexity, respectively. Our characterization of convex contours will then follow naturally from these geometric interpretations.
\begin{defn}[Monotonicity]
$f: \mathcal{D} \subset \mathds{R} \to \mathds{R}$ is called (strictly) monotonically decreasing if $f(t_{i_1}) (>) \geq  f(t_{i_2})$ for all $t_{i_1} < t_{i_2}$ from $\mathcal{D}$. $f$ is (strictly) monotonically increasing if $-f$ is (strictly) monotonically decreasing. %
\end{defn}
The following characterization of monotonicity by sign consistency follows from direct computations:
\begin{lem}\label{lem:mono}
  	Let $f: \{t_{1}, t_{2}, \dots, t_{n} \} \to \mathds{R}$ with $t_{i} < t_{i+1}$ for all $i \in (1:n-1)$ and 
  	\begin{equation*}
  		M^f := 	\begin{bmatrix}
  			f(t_{1}) & 1\\
  			f(t_{2}) & 1 \\
  			\vdots & \vdots \\
  		 f(t_n) & 1
  		\end{bmatrix}
  	\end{equation*}
  	Then, the following are equivalent:
\begin{lemenum}
  		\item $f$ is (strictly) monotonically decreasing. 
  		\item $M^f_{[2]} (>) \geq 0$. 
  		\item For all $i \in (1:n-1)$ it holds that \label{item:mono_delta}
  		\begin{equation*}
  		 \det \begin{bmatrix}
  				f(t_i) & 1\\
  				f(t_{i+1}) & 1
  			\end{bmatrix} (>) \geq 0
  		\end{equation*}
\end{lemenum}
\end{lem}
Alternatively, \cref{lem:mono} can also be verified by noticing that a function is monotone if and only if it crosses any value in $\mathds{R}$ at most once and cannot remain in a value under the additional strictness assumption. As this property is invariant with respect to scaling and translation, this translates to
\begin{equation*}
\forall u \in \mathds{R}^2\setminus \{0\}:	(\variz{u_1 f + u_2 \mathbf{1}})\; \vari{u_1 f + u_2 \mathbf{1}}\leq 1,
\end{equation*} 
which by \cref{item:SC_full_rank,item:SC_low_rank} leads to the same conclusion. Moreover, \cref{prop:karlin_scm} in case of $m=2$ can be recovered by from \cref{lem:mono} by noticing that 
if the second column of $X \in \mathds{R}^{n \times 2}$ consists of elements with the same strict sign, then by \cref{eq:Cauchy_Binet}
 \begin{equation}
 	X = \begin{bmatrix}
 		x_{12} &  &\\
 		& \ddots & \\
 		& & x_{n2}
 	\end{bmatrix} \begin{bmatrix}
 	\frac{x_{11}}{x_{12}} & 1\\
 	\vdots & \vdots \\
 	\frac{x_{n1}}{x_{n2}} & 1
 \end{bmatrix} \in \text{(S)SC}_2 \label{eq:fact}
 \end{equation}
 if and only if the second factor is $\text{(S)SC}_2$. Interpreting this second factor as the matrix $M^f$ in \cref{lem:mono}, it follows from \cref{item:mono_delta} that it is enough to verify that only consecutive $2$-minors share the same sign. This, however, is equivalent to checking the consecutive $2$-minors of $X$ itself. 
 
 Next, we will move on the case of $m=3$ and its links to convexity. 
 \begin{defn}[Convexity/Concavity]\label{def:cvx}
	Let $\mathcal{D} := \{t_1,\dots,t_n\}$. Then, $f: \mathcal{D} \to \mathds{R}$ is \emph{(strictly) convex} if for all fixed $\tau \in \mathcal{D}$
	\begin{equation}
s(t,\tau) := \frac{f(t) - f(\tau)}{t-\tau} = \frac{f(\tau) - f(t)}{\tau-t} 
	 \label{eq:def_cvx_seq}
	\end{equation}
	is (strictly) monotonically increasing in $t$ on $\mathcal{D} \setminus \{\tau\}$. $f$ is called \emph{(strictly) concave} if $-f$ is (strictly) convex. 
\end{defn}
Note that this definition of convexity via the so-called \emph{slope function} $s(t,\tau)$ is a well-known equivalence in the theory of continuous convex functions \cite[Proposition~1.1.4]{hiriart2013convex}. Moreover, by \cite[Proposition~5.3.1]{hiriart2013convex}, it follows that the piecewise-linear continuous extension $\bar{f}: [t_1,t_n] \to \mathds{R}$ of $f$ defined by
\begin{equation}
	\bar{f}(t) := f(t_i) + \frac{f(t_{i+1}) - f(t_i)}{t_{i+1} - t_i}(t-t_i), t_i \leq t \leq t_{i+1} \label{eq:f_ext}
\end{equation}
is convex if and only if its right-derivatives are monotonically increasing. However, by the piecewise-linearity, these derivatives correspond to $s(t_{i+1},t_i)$. Expressing the monotonicity of the slope function $s(t,\tau)$ via \cref{lem:mono}, gives the following characterizations in terms of sign-consistency:
\begin{lem}\label{lem:convex}
	Let $f: \{t_{1}, t_{2}, \dots, t_{n} \} \to \mathds{R}$ with $t_{i} < t_{i+1}$ for all $i \in (1:n-1)$ and 
	\begin{equation*}
		M^f := 	\begin{bmatrix}
			t_{1}  & f(t_{1}) & 1 \\
			t_{2}  & f(t_{2}) & 1 \\
			\vdots & \vdots & \vdots \\
			t_{n}  & f(t_{n}) & 1 \\
		\end{bmatrix}
	\end{equation*}
	Then, the following are equivalent:
	\begin{lemenum}
		\item $f$ is (strictly) convex. \label{item:cvx_f}
		\item $\bar{f}$ in \cref{eq:f_ext} is convex (and no three points of $\{(t_i,f(t_i)): t_i \in \mathcal{D}\}$ are co-linear).  \label{item:bar_f}
		\item $M^f_{[3]} (>) \geq 0$.  \label{item:cvx_comp}
		\item For all $i \in (1:n-2)$ it holds that \label{item:cvx_det}
		\begin{equation*}
			 \det \begin{bmatrix}
				t_{i}  & f(t_{i}) & 1 \\
			t_{i+1}  & f(t_{i+1}) & 1 \\
			t_{i+2}  & f(t_{i+2}) & 1	
			\end{bmatrix} (>) \geq 0.
		\end{equation*}
	\end{lemenum}
\end{lem}
Using \cref{item:SC_full_rank,item:SC_low_rank}, it can be seen that $f$ is either convex or concave if and only if each line $H := \{(x,y): \; L_\alpha(x,y) := \alpha_1 + \alpha_2 x + \alpha_3 y = 0\}$, $\alpha \in \mathds{R}^3$, is crossed at most twice by the curve $\gamma: \{t_1,\dots,t_n\} \to \mathds{R}^2$ with $\gamma(t_i) := (t_i,f(t_i))$, $i \in (1:n)$ and no more than two points of $\gamma$ can be co-linear. Thus, drawing the connection to the classical definition of convexity/concavity. In terms of variation bounding, this reads as
\begin{equation}
\forall \alpha \in \mathds{R}^3: \; \vari{L_\alpha(\gamma)} \; (\variz{L_\alpha(\gamma)}) \leq 2. \label{eq:cvx_var}
\end{equation}
Again \cref{prop:karlin_scm}, in case of $m=3$, can be recovered from \cref{lem:convex} by applying the analogues factorization argument as in \cref{eq:fact}.  

\subsection{Convex Contours}
Next, we will extend theses observations to establish our first main result on the characterization of so-called (strictly) convex contours, which we define directly in terms of our variation notions: 
\begin{defn}\label{defn:convc}
	A sequentially $T$-periodic curve $\gamma: \mathds{Z} \to \mathds{R}^2$ is called a \emph{convex contour} ($\gamma \in \cc{T}$) if 
	for all $\alpha \in \mathds{R}^3 \setminus \{0\}$ it holds that $\Sm_c[\alpha_1	\gamma_1+\alpha_2\gamma_2 + \alpha_3] \leq 2$. $\gamma$ is said to be a \emph{strictly convex contour ($\gamma \in \scc{T}$)} if $\Sm_c$ can be replaced by $\Sp_c$. 
\end{defn}
Visually, if $\gamma \in \cc{T}$ does not lie on a line, then the polygon
\begin{equation}
	\mathcal{P}_\gamma(t) := \begin{bmatrix}
		\gamma_1(\floor{t}) + (t-\floor{t})\gamma_1(\ceil{t}) \\
		\gamma_2(\floor{t}) + (t-\floor{t})\gamma_2(\ceil{t})
	\end{bmatrix}, \quad t \in [0,T) \label{eq:convc}
\end{equation} 
that results from connecting $\gamma(0),\gamma(1),\dots, \gamma(T-1),\gamma(0)$ sequentially must be the boundary of a convex set in $\mathds{R}^2$ and the curve must be \emph{simple} (i.e., non-intersecting apart from consecutive points $\mathcal{P}_\gamma(t) = \mathcal{P}_\gamma(t+1)$). In the strict case, it is additionally required that no three vertices of the polygon can be co-linear (see~\Cref{fig:third_order_cc} in \Cref{sec:LTI_ex}). 

Using \cref{prop:sc_k_mat_vb_m,lem:convex}, sequentially convex contours can be tractably characterized as follows:
\begin{thm} \label{prop:convc_ct}
	Let $\gamma: \mathds{Z} \to \mathds{R}^2$ be $T$-periodic with $T\geq 4$, 
	\begin{equation}
		M^\gamma := \begin{bmatrix}
			\gamma_1(0) & \gamma_2(0) & 1\\
			\gamma_1(1) & \gamma_2(1) & 1\\
			\vdots & \vdots & \vdots\\
			\gamma_1(T-1) & \gamma_2(T-1) & 1
		\end{bmatrix}, \label{eq:M_mat}
	\end{equation}
	and $\tilde{\gamma}: \mathds{Z} \to \mathds{R}^2$ be the $\tilde{T}$-periodic sequence that results from deleting all points with indices $\mathcal{I}_0 := \{t \in \mathds{Z}: \Delta \gamma(t) = 0\}$ from $\gamma$. If $\rk(M^\gamma) = 3$, then the following are equivalent:
	\begin{thmenum}
		\item $\gamma \in \text{(S)}\cc{T}$. \label{item:prop_CC}
		\item \label{item:prop_compound} $\compound{M^\gamma}{3} \in \text{(S)}\sgc{3}$. 
		\item All determinants \label{item:prop_minor}
		\begin{equation} \label{eq:det_gamma}
			\det\begin{bmatrix}
				 \gamma_1(t_1) & \gamma_2(t_1) & 1\\
				\gamma_1(t_2) & \gamma_2(t_2) & 1\\
				\gamma_1(t_3) & \gamma_2(t_3) & 1
			\end{bmatrix}, t_1 < t_2 < t_3 < t_1 + T
		\end{equation}
		share the same (strict) sign.
		\item \label{item:prop_polygon} $P_\gamma$ is simple such that the set enclosed by $P_\gamma([0,T))$ is convex (and no three points of $\gamma(0:T-1)$ are co-linear). 
		\item  All determinants \label{item:prop_PM}
		\begin{equation} \label{eq:det_gamma_consec}
			\det \begin{bmatrix}
				\Delta \tilde{\gamma}_1(t) & \Delta \tilde{\gamma}_2(t)\\
				\Delta \tilde{\gamma}_1(t+1) & \Delta \tilde{\gamma}_2(t+1) 
			\end{bmatrix}, \; t \in (0,\tilde{T}-1)
		\end{equation}
		share the same (strict) sign and $\tilde{\gamma}_1, \tilde{\gamma}_2 \in \text{(S)}\pmu{\tilde{T}}$.
	\end{thmenum}
If $\rk(M^\gamma) = 2$, then $\gamma \in \cc{T}$ if and only if $\gamma_1, \gamma_2 \in \pmu{T}$. 
\end{thm}
Note that the requirement for using $\tilde{\gamma}$ in  \cref{item:prop_PM} cannot be removed. An example for this is the following
\begin{align*}
M^\gamma := 	\begin{bmatrix}
		\gamma_1(0) & \gamma_2(0) & 1\\
		 \gamma_1(1) & \gamma_2(1) & 1\\
		\gamma_1(2) & \gamma_2(2) & 1\\
		\gamma_1(3) & \gamma_2(3) & 1\\
		\gamma_1(4) & \gamma_2(4) & 1\\
		\gamma_1(5) & \gamma_2(5) & 1\\
		\gamma_1(6) & \gamma_2(6) & 1\\
	\end{bmatrix} := \begin{bmatrix}
	0 & 0 & 1\\
	1 & 0 & 1\\
	1 & 0 & 1\\
	1 &  1 & 1\\
	1  & 1 & 1\\
	0.5 & 0 & 1\\
	0.5 & 0 & 1\\
\end{bmatrix}
\end{align*}
where $\gamma_1,\gamma_2 \in \pmu{7}$. The corresponding determinants defined in \cref{eq:det_gamma_consec} are zero, but $\varic{M^\gamma \alpha} = 4$ for $\alpha = \begin{bmatrix}
	 -1 & 1 & 0.25
\end{bmatrix}^\transp$. Deletion of consecutive repetitive points in $\gamma$ yields a new $4$-periodic $\tilde{\gamma}$ with
\begin{align*}
\begin{bmatrix}
	\tilde{\gamma}_1(0) & \tilde{\gamma}_2(0)\\
	\tilde{\gamma}_1(1) & \tilde{\gamma}_2(1)\\
	\tilde{\gamma}_1(2) & \tilde{\gamma}_2(2)\\
	\tilde{\gamma}_1(3) & \tilde{\gamma}_2(3)\\
			\end{bmatrix} := \begin{bmatrix}
	0 & 0\\
	1 & 0\\
	1  & 1\\
	0.5 & 0\\
	\end{bmatrix}
\end{align*}
where this time
\begin{align*}
	\det \begin{bmatrix}
		\Delta \tilde{\gamma}_1(0) & \Delta \tilde{\gamma}_2(0)\\
		\Delta \tilde{\gamma}_1(1) & \Delta \tilde{\gamma}_2(1) 
	\end{bmatrix} = 1, \; \det \begin{bmatrix}
	\Delta \tilde{\gamma}_1(2) & \Delta \tilde{\gamma}_2(2)\\
	\Delta \tilde{\gamma}_1(3) & \Delta \tilde{\gamma}_2(3) 
\end{bmatrix} = -0.5.
\end{align*}
\begin{rem}\label{rem:tilde_gamma}
	From the proof of \cref{prop:convc_ct}, it can be deducted that if $\mathcal{I}_+ := \{i \in (0:T-1): \; \Delta \gamma_1(i) > 0\} = (T_0:T_p)$ and $\mathcal{I}_- := \{ i \in (0:T-1): \; \Delta \gamma_1(i) < 0\} = (T_b:T_n)$, $T_p < T_b$ and $\vari{\Delta \gamma_2(T_p+1:T_b-1)} = \vari{\Delta \gamma_2(T_p+1:T_b-1)}  = 0$, then $\tilde{\gamma}$ can be replaced by $\gamma$. In particular, this is implied by $\gamma_1 \in \spmu{T}$, because then $T_b \leq T_p + 2$ due to \cref{lem:pmu_delta}. %
\end{rem}

Further, from the proof of \cref{prop:convc_ct}, it can also be seen that the difference between positive and negative signs in \cref{eq:det_gamma} is due to the \emph{orientation} of $\mathcal{P}_\gamma$, i.e., $\mathcal{P}_\gamma$ is \emph{positively (counter-clockwise)/negatively (clock-wise) oriented} if and only if the determinants in \cref{eq:det_gamma} are nonnegative/nonpositive. 

Finally, by the same factorization as for $m=2$, \cref{prop:convc_ct} provides a direct extension of \cref{prop:karlin_scm} for the case of $m=3$, which we will use to characterize $\Conv{g} \in \cvb{2}$. However, this also raises the open question of how to geometrically extend these results to $m > 3$. 



 





 




